Multi-Variant Execution at the Edge

Edge-cloud computing offloads parts of the computations that traditionally occurs in the cloud to edge nodes,e.g., CDN servers, in order to get closer to the users and reduce latency. To improve performance even further, WebAssembly is increasingly used in this context. Edge-cloud computing providers, such as Fastly or Cloudflare, let their clients deploy stateless services in the form of WebAssembly binaries, which are then translated to machine code and sandboxed for a safe execution at the edge. In this context, we propose a technique that (i) automatically diversifies WebAssembly binaries that are deployed to the edge and (ii) randomizes execution paths at runtime, turning the execution of the services into a moving target. Given a service tobe deployed at the edge, we automatically synthesize functionally equivalent variants for the functions that implement the service.All the variants are then wrapped into a single multivariant WebAssembly binary. When the service endpoint is executed,every time a function is invoked, one of its variants is randomly selected. We implement this technique in the MEWE tool and we validate it with 7 services for cryptography and QR encoding. MEWE generates multivariant binaries that embed hundreds of function variants. We execute the multivariant binaries on the worldwide edge platform provided by Fastly. We show that,at runtime, the multivariant exhibit a remarkable diversity ofexecution traces, across the whole edge platform.

==> diagrams/ex_model.tex <==
%% Creator: Inkscape 1.1 (c4e8f9e, 2021-05-24), www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'ex_model.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{709.5bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.59936575)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{ex_model.pdf}}%
    \put(0.32507344,0.57147184){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Multivariant execution at the Edge\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=2]{ex_model.pdf}}%
    \put(0.02947456,0.50880353){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Client computer\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=3]{ex_model.pdf}}%
    \put(0.2898636,0.50880353){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Closest Edge Node\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=4]{ex_model.pdf}}%
    \put(0.52269801,0.50880353){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Multivariant binary\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=5]{ex_model.pdf}}%
    \put(0.71081782,0.50880353){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Random generator\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=6]{ex_model.pdf}}%
    \put(0.92292744,0.50880353){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Variant\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=7]{ex_model.pdf}}%
    \put(0.12370185,0.43627938){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}HTTP request to the service\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=8]{ex_model.pdf}}%
    \put(0.3814834,0.38421074){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Execute endpoint harness\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=9]{ex_model.pdf}}%
    \put(0.65258421,0.33214213){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Execute\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=10]{ex_model.pdf}}%
    \put(0.61045944,0.28007349){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Variant discriminator\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=11]{ex_model.pdf}}%
    \put(0.61969433,0.22800486){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Execute variant based on the discriminator\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=12]{ex_model.pdf}}%
    \put(0.7443067,0.17593623){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Result\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=13]{ex_model.pdf}}%
    \put(0.3830338,0.12386762){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}HTTP Response + Result\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=14]{ex_model.pdf}}%
    \put(0.10860319,0.07179899){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}HTTP response from the service\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=15]{ex_model.pdf}}%
  \end{picture}%
\endgroup%


==> notes/notes.tex <==
E. Wen \etal. \cite{eWenWasmachine} and Kishore \etal. \cite{10.1145/3423211.3425680} present  Wasmachine as an OS kernel to evaluate Wasm based programs. The compiling of AOT Wasm programs is implemented as a LLVM frontend and linked with the OS proxy implementation. The OS proxy is implemented in Rust taking into account the countermeasures for memory vulnerabilities. Since the final compilation is meant to run in the kernel space, it gains a 21\% performance over native counterparts. Wasmachine uses LLVM, this means that a large number of optimisations can be applied, reaching more performance that the one obtained by V8. The using of LLVM, allows the deploy of the programs in heterogeneous architectures, and here is where the “Edge” plays a role. The main difference with out work, is that they evaluate the feasibility of the tool but it is not evaluated in a real service like Fastly, so there is no evaluation in different CPU architectures for example. Second, there is no mention to Lucet which has the same idea after all.

\todo{Add aWsm paper here as a previous work for Sledge}

Sledge \cite{10.1145/3423211.3425680} compiles takes Wasm binaries as input an provides a compilation to LLVM intermediate representation. It relies on LLVM backend to perform optimization for architectures. Existing Wasm runtimes can exhibit significant overhead in properly sandboxing code, Sledge uses AoT compiler for Wasm to LLVM to leverage the overhead to native performance. Sledge system leverages the Wasm security model to enable exeution of multiple unstrusted modules in the same process, \todo{Add comparison with Lucet here}. However, Sledge adds a bound checking overhead since the memory accesses need to be done calling from a function inside a module to another. 


==> notes/old.tex <==
\paragraph{Backend modification}
The Rustc compiler can be configured to use a specific LLVM toolchain, i.e. frontends, backends, optimization passes and linker.
As mentioned in CROW's paper~\cite{CabreraArteaga2020CROWCD}, the usage of the standard LLVM backend for \wasm can remove some variants due to enabled peephole optimizations. 
To prevent this removal of variants, we replaced the LLVM backend in our pipeiline  with the one provided by CROW's authors.



%The goal of \tool is to augment at compile time a WebAssembly program with variants.
%We define a variant as an alternative execution path that is semantically equivalent to the original one but with different instructions.
%This way, through this augmentation, the program presents a MTD behavior whose main execution path is randomly selected at runtime.

It should be noted that CROW cannot diversify all functions inside a binary. 
CROW is oblivious to the memory model of a program code and thus, codes interacting with the memory will not be used to generate variants.




\todo{Change, speak in terms of static path preservation. }

The methodology for RQ1 shown in \autoref{diagram:methodrq1} works as follows. First, we pass a module to CROW as it generates bytecode variants of the original module (Step \step{1}). Each variant is then compiled into its own corresponding Wasm module using the \texttt{rustc+CROW backend} (Step \step{2}). 
We combine different variant modules with the original one into a single package and compile it using Cranelift so that it can be deployed on Fastly's infrastructure (Step \step{3}). 
Finally, we compare the machine codes of the variants embedded in a single module to make sure that they are different (Step \step{4}). 
If they are not, this means the compilation chain has removed what made them unique and we discard this module from our experiment. 
It should be noted that we use the most aggressive optimizations possible with Cranelift so that we are keeping the modules where we are sure that the variants are preserved. 

To provide an even better understanding of our pipeline, let us analyze the example in the diagram. Hypothetically, CROW generates 2 variants for the original module in \step{1}. Rustc compiles the 2 bytecode modules, generating 2 unique Wasm packages \step{2}. Two symmetric pairs can be built \step{3} from the 2 generated Wasm binaries. Then, for each pair, the Cranelift compiler generates the corresponding machine code. In one pair, the generated machine codes are equal even when the original pair is formed by two different Wasm codes so we discard it \step{4}. For the other, the generated machine codes are different and we keep it. In the end, we have a 50\% preservation rate as variants in one module out of two were preserved.  


\todo{Fix table,  x86 instead of machine code}


For each module inside the projects, we perform the workflow described in \autoref{diagram:methodrq1}. We collect all the Wasm variant pairs for the diversified functions inside the module. We then calculate the preservation rate on the generated x86 machine code with Cranelift. 



%Assumptions:

%- The analysis phase can be done from everywhere, So, moving target network wont work, since the application is deployed in a world scale. Besides, the main idea of the Edge is to get rid of the latency, this technique will increase the latency.

%- Since the platform is heterogeneous, there is a natural protection according to Holland \etal. But it is not enough

%- FaaS is small enough to embed the multiversion in the same binary

%- The model attack is a combination C of parameters that can trigger a bad behavior. The developer does not know C, then, C should not work for all nodes. If developer already know C, the combination should not work more than one time between the discovery and the successful redeployment.

%- The removal of latency, allows the study of time side-channel close to the client. \todo{Check !}. If there is time side-channel attacks, check that the generated diversification is less than the natural latency and greater than the lapse between regional classification.


\begin{comment}
 

\lstdefinestyle{nccode}{
    numbers=none,
    firstnumber=2,
    stepnumber=1,
    numbersep=10pt,
    tabsize=4, 
    showspaces=false,
    breaklines=true, 
    showstringspaces=false,
    moredelim=**[is][\btHL]{`}{`},
    moredelim=**[is][{\btHL[fill=black!10]}]{`}{`},
    moredelim=**[is][{\btHL[fill=celadon!40]}]{!}{!}
}
\lstset{
    language=WAT,
    style=nccode,
    basicstyle=\footnotesize\ttfamily,
    columns=fullflexible,
    breaklines=true
}
\begin{code}
\noindent\begin{minipage}[b]{0.9\linewidth}
    \captionof{lstlisting}{Constant operand splitting.}\label{add:prevalence_example}
    \noindent\rule{\linewidth}{0.4pt}
    \begin{minipage}[t]{0.45\linewidth}
        \begin{lstlisting}
i32.const 9                                           
i32.add                                                
i32.const 4                                          
i32.add                                               
i32.const 12                                        
i32.add                                              
i32.const 7                                     å     
i32.add  
        \end{lstlisting}
    \end{minipage}%
    \hfill\noindent\begin{minipage}[t]{0.45\linewidth}
       
        \begin{lstlisting}
i32.const 13
i32.add
i32.const 8
i32.add
i32.const 1
i32.add
i32.const 10
i32.add
        \end{lstlisting}
    \end{minipage}
\end{minipage}
\end{code}


\begin{code}
\noindent\begin{minipage}[b]{0.9\linewidth}
    \captionof{lstlisting}{Inversion of operations.}\label{add:prevalence_example}
    \noindent\rule{\linewidth}{0.4pt}
    \begin{minipage}[t]{0.45\linewidth}
        \begin{lstlisting}
i32.const -<n>
i32.sub
        \end{lstlisting}
    \end{minipage}%
    \hfill\noindent\begin{minipage}[t]{0.45\linewidth}
       
        \begin{lstlisting}
i32.const <n>
i32.add
        \end{lstlisting}
    \end{minipage}
\end{minipage}
\end{code}



\begin{code}
\noindent\begin{minipage}[b]{0.9\linewidth}
    \captionof{lstlisting}{Multiplication overflow.}\label{add:prevalence_example}
    \noindent\rule{\linewidth}{0.4pt}
    \begin{minipage}[t]{0.45\linewidth}
        \begin{lstlisting}
  i32.const -1931544174
  i32.mul
  i32.const 109653155
  i32.mul
        \end{lstlisting}
    \end{minipage}%
    \hfill\noindent\begin{minipage}[t]{0.45\linewidth}
       
        \begin{lstlisting}
  i32.const -10
  
  
  i32.mul
        \end{lstlisting}
    \end{minipage}
\end{minipage}
\end{code}





\begin{code}
\noindent\begin{minipage}[b]{0.9\linewidth}
    \captionof{lstlisting}{Multiplication overflow.}\label{add:prevalence_example}
    \noindent\rule{\linewidth}{0.4pt}
    \begin{minipage}[t]{0.45\linewidth}
        \begin{lstlisting}
  i32.const -1931544174
  i32.mul
  i32.const 109653155
  i32.mul
        \end{lstlisting}
    \end{minipage}%
    \hfill\noindent\begin{minipage}[t]{0.45\linewidth}
       
        \begin{lstlisting}
  i32.const -10
  
  
  i32.mul
        \end{lstlisting}
    \end{minipage}
\end{minipage}
\end{code}


\end{comment}

\subsection{Definitions (to be removed)}
In this subsection we define the key concepts for that we use along the paper. 

\todo{Define on the fly.}
\todo{Define multivariant call graph in term of variants and dispatchers.}

\begin{definition}{Unique Wasm variants, $W(F)$:}\label{def:W}
    Let $F$ be a program function, $W(F)$ a set of Wasm binaries  such that each binaryis a unique function variant generated by CROW from a function $F$.
\end{definition}

\begin{definition}{Binary translation function ,$C$:}\label{def:compiler}
    Let $w$ be a Wasm module, $x$ an x86 machine code and $C: Wasm \rightarrow x86 $ a translation function. $C$ is a binary translation function if it generates the corresponding x86 machine code $x$ for the Wasm binary$w$ such that $C(w) = x$.
\end{definition}

\begin{definition}{Unique x86 variants , $X(F)$:}\label{def:X}
    Let $F$ be a function, $W$ the Unique Wasm variants set according to \autoref{def:W} and $C$ a compiler function according to \autoref{def:compiler}. We define $X$ = \{ $x, C(w) = x, w \in W$ \} as the set of unique x86 machines codes that can be generated from $W$.
\end{definition}



\begin{definition}{Multivariant binary:}\label{def:EP}
    Let $F$ a function and $W$ its collection of variants. The multivariant binary $M$ is the binarythat packages all function variants in it. Notice that the concept of multivariant could be applied to any code representation. We use multivariant binary indistinctly for any code representation, for example, " multivariant Wasm  binary".
\end{definition}

\begin{definition}{Call Graph (CG):}\label{def:EP}
    We use an approximation of the traditional definition of Call Graph from Aho \etal \citationneeded. We only take into account the functions that executes in a static analysis of the source code. 
\end{definition}

\begin{definition}{Execution traces:}\label{def:DEP}
    Let $F$ an endpoint function in the Edge service. The execution path $S = F_1, F_2, ... F_n$ is the trace of the function in the Call Graph of the binary, executed from the request to the response to the client. 
\end{definition}



In 2019, it was accepted as the fourth official language for the web \cite{WebAssemblyCoreSpecification}.
Moreover, \wasm is used in standalone environments beyond the web context \cite{2021arXiv210212730N, 1244493Jacobsson, WARDuino2019,eWenWasmachine,10.1145/3423211.3425680}.
Nowadays, languages such as C/C++, C\#, Go and Rust can be compiled to Wasm \cite{hilbig2021empirical}. 
Since version 9.0, LLVM added the \wasm backend as a platform for code generation, making possible the generation of Wasm code from any LLVM frontend.

\begin{metric}{Deployment speed:}\label{metric:size}
For a given binary, the time passed between uploading the binary to the Fastly Edge infrastructure to its deployment to the edge nodes is the deployment time. 
We measure the deployment time for both kind of binaries, original and multivariant.
\end{metric}

% Define deployment time
Since the deployment time is correlated with the size of the binary, we collect Metric \autoref{metric:size} only for the largest multivariant binary.
The largest multivariant binary is generated for the endpoint \textbf{generate\_qr\_str}.
The original and multivariant binaries have 3Mb and 13Mb of size respectively.

% How to collect the times
We collect 500 deployment times for each.
To avoid the possible jitter in the network, we collect the deployment time from 4 different edge nodes in 4 different timezones.
The total number of collected deployment times is $2\times 4\times 500$.

\todo{TBD, should we mention the protocol to collect the deplyment time ? }


% Worst case
The largest size of a multivariant binary is 13Mb for the original binary named \textbf{generate\_qr\_str}, which has a size of 3Mb.
In this case, the deployment time is increased by approx. 1 second from the original mean deployment time of 12.07s.
These values are in concordance with the average time reported by Fastly for its deployment time, which is 13s.
Therefore, the deployment time is not increased by the multivariant binaries created by \tool.


%\todo{Add A Stackelberg Game and Markov Modeling of Moving Target Defense as well }\url{https://www.researchgate.net/publication/320203887_A_Stackelberg_Game_and_Markov_Modeling_of_Moving_Target_Defense}
%\todo{https://arxiv.org/pdf/1905.13293.pdf}

%The main difference with currently available MTD systems is that \tool performs the multivariant system in an automated way. 


%Serverless approaches

% Standalone interpreters for \wasm

% \todo{Add aWsm paper here as   a previous work for Sledge}



%\todo{ wasmachine -> Virtual machine execution for wearables based on
%WebAssembly. \cite{1244493Jacobsson} }




%Benchmark studies, feasibility and Wasm in Edge approaches%

%This is more a motivation to the usage of Wasm

%\todo{Considering WebAssembly Containers for Edge Computing on Hardware-Constrained IoT Devices 2020 master thesis Blekinge \cite{Napieralla2020}.}





% 2014



%Torquato, Matheus, and Marco Vieira. "Moving target defense in cloud computing: A systematic mapping study." Computers & Security 92 (2020): 101742.


%\todo{TBD, multivariatn execution means to execute several variants at the same time to detect anomalies. 
%}

%\textbf{Moving Target Defense and security related}



We collect $64\times100$ execution traces because the deplyment speed of our experimentation platform is in average 13s. 
In an hypothetical case of attack, if it detected a patch or even the disconnection of the service can be done in 13s.
This makes unreallistic to collect the traces in more than 13s.

\subsection{Moving Target Defense}

\todo{purpose of these two paragraphs is not clear. Do we need a subsection about MTD?}

% Intro and benefits
Moving Target Defense (MTD) for software was first proposed   as a collection of techniques that aim to improve security of a system by constantly moving its vulnerable components \cite{MTDNationalCyberLaep}.
Usually, MTD techniques revolve around changing system inputs and configurations to reduce attack surfaces . 
This increases uncertainty for attackers and makes their attacks more difficult. 
Ultimately, potential attackers cannot hit what they cannot see. 

% Example
MTD can be implemented in different ways, including via dynamic runtime platforms \cite{10.1145/3318216.3363338}. 
Segupta \etal illustrated how a dynamic MTD system \cite{10.5555/3091125.3091155} can be applied to different technology stacks.
Using this technique, the authors illustrated that some CVE related to specific database engines can be avoided.
Notice that MTD implementation should be practical, in the previous example, the challenging part is to maintain the synchronization between the different implementations.


\lstset{
    language=CURL,
    style=nccode,
    basicstyle=\footnotesize\ttfamily,
    columns=fullflexible,
    breaklines=true
}

\begin{code}
\noindent\begin{minipage}[b]{0.9\linewidth}
    
    \begin{minipage}[t]{1\linewidth}
        \begin{lstlisting}
< HTTP/2 200 
< xpop: BMA
< xpophash: 1293274507
< xtime: 1999109
!< xpath: !
! [1859, 1836, 1765, 1767, 1800, 1767, 1801, !
! 1767, 1799, 1767, 1800, 1767, 1801, 1767, !
! 1801, 1767, 1801, 1767, 1800, 1767, 1799, !
! 1767, 1800, 1767, 1799, 1767, 1799, 1767, !
! 1801, 1767, 1799, 1767, 1801, 1767, 1799, !
! 1767, 1799, 1767, 1801, 1767, 1800, 1767, !
! 1799, 1767, 1801, 1767, 1801, 1767, 1799, !
! 1767, 1801, 1767, 1799, 1767, 1800, 1767, 1801]!
< date: Thu, 03 Jun 2021 14:33:36 GMT
< content-length: 74
< 
{ [74 bytes data]
* Connection #0 to host totally-devoted-krill.edgecompute.app left intact
* Closing connection 0
        \end{lstlisting}
    \end{minipage}%
    
    \noindent\rule{\linewidth}{0.4pt}
    \captionof{lstlisting}{Execution path retrieval example for one query to one of the executed endpoints. The execution path is highlighted in the header of the response in green color. Each function is annotated with an unique id.}\label{retrieval_example}
\end{minipage}
\end{code}


\todo{the end of the paragraph is very hard to understand}
This cloud model \todo{what is 'this cloud model'?} is done at or near the customer’s physical location instead of relying on the cloud at one of a dozen data centers to do all the work. 
Literally, this has a geographic meaning. 
Every time an Edge endpoint is executed, the closest node is the one responding.

\todo{how is this first sentence related to the previous paragraph?}


\todo{Javier: TBD, lets avoid to talk about security here}
% Swivel and Spectre
On the other hand, even when \wasm is a performant way to deploy services at the Edge \cite{10.1145/3302505.3310084}, Narayan \etal \cite{2021arXiv210212730N} remarked, it is not exempt of vulnerabilities.
Spectre attacks can bypass Wasm's isolation.
A malicious deployed Wasm can use Spectre to break out of the sandbox to leak another process memory by miss-training the speculative execution of the Edge node CPU.
v


\begin{figure}
    \includegraphics[width=0.8\linewidth]{diagrams/RQ1.pdf}
    \caption{Example of a Multivariant Call Graph and its preservation during x86 compilation. From left to right: original binary CG, Wasm multivariant binary MCG generated by \tool and the x86 multivariant binary MCG that is deployed after Lucet compiles the Wasm multivariant to machine code.}
    \label{diag:rq1}
\end{figure}


Machine learning models can be deployed to the Edge for faster classification near to devices \cite{https://doi.org/10.1002/spe.2944}.
These models are not exempt of vulnerabilities.
Roy \etal \cite{10.1145/3318216.3363338} proposed a moving target defense against adversarial machine learning.
Their technique shows that switching among machine learning algorithms can be used to defend against boundedly rational adversary without sacrificing performance.
In addition, they remarked that adding more randomness to the algorithm variants achieve better defense.
\tool adds a remarkable amount if different execution paths in an automated way that a multivariant Wasm module can execute and can be used to increment of uncertainty for adversarial-based attacks.


==> old.tex <==


\subsection{Related work on Moving Target Defense}
% MTD with natural diversity
There are significant previous work in the space of moving target defenses. 
Taguinod \etal \cite{taguinod2015toward} and Christodorescu \etal \cite{Christodorescu2011}  proposed to diversify different layers of web applications by using preexisting diversity. In the same machine, they constantly switch the application's logic between SQL database engines and web servers implemented in different languages such as PHP, Python, Java and Ruby.
Similarly, Roy \etal \cite{10.1145/3318216.3363338} harnessed diverse  machine learning algorithms for the same classification task at the Edge, creating a moving target defense against adversarial learning attacks.
These works try to break reconnaisance stages from potential attackers.
The usage of preexisting variants limits the diversification space.
\tool creates artificial diversity instead of using preexisting variants.
\tool is agnostic to the platform where the service is deployed and no manpower is needed to implement a rotational stack system.
Besides, \tool operates at a worldwide scale edge-cloud computing platform.

% Diversification and randomization at low-level
Different layers of software stacks can be diversified \cite{OkhraviBlur14}. In particular for dynamic  platforms  techniques,
Holland \etal \cite{10.1145/1055626.1055632}, Okhravi \etal \cite{OKHRAVI201230} and  Wang \etal \cite{259693} proposed to use preexisting diversity to achieve implicit protection for MTD. They proposed to use different virtual machines configurations to create a diverse set of ISAs.
Besides, Caballero \etal \cite{DBLP:conf/ndss/CaballeroKSW08} 
also proposed to use preexisting diversity over TIER-1 ISP layers to prevent monoculture over network router implementations. Edge-cloud computing platforms are heterogeneus architectures by definition, therefore, they have an implicit protection.
However, as previous works remarked, it does not protect yet against application-level attacks.
\tool is the counterpart, it provides runtime diversification and provides a practical MTD for edge-cloud platforms, at software level.









\paragraph{Backend modification}
The Rustc compiler can be configured to use a specific LLVM toolchain, i.e. frontends, backends, optimization passes and linker.
As mentioned in CROW's paper~\cite{CabreraArteaga2020CROWCD}, the usage of the standard LLVM backend for \wasm can remove some variants due to enabled peephole optimizations. 
To prevent this removal of variants, we replaced the LLVM backend in our pipeiline  with the one provided by CROW's authors.



%The goal of \tool is to augment at compile time a WebAssembly program with variants.
%We define a variant as an alternative execution path that is semantically equivalent to the original one but with different instructions.
%This way, through this augmentation, the program presents a MTD behavior whose main execution path is randomly selected at runtime.

It should be noted that CROW cannot diversify all functions inside a binary. 
CROW is oblivious to the memory model of a program code and thus, codes interacting with the memory will not be used to generate variants.




\todo{Change, speak in terms of static path preservation. }

The methodology for RQ1 shown in \autoref{diagram:methodrq1} works as follows. First, we pass a module to CROW as it generates bytecode variants of the original module (Step \step{1}). Each variant is then compiled into its own corresponding Wasm module using the \texttt{rustc+CROW backend} (Step \step{2}). 
We combine different variant modules with the original one into a single package and compile it using Cranelift so that it can be deployed on Fastly's infrastructure (Step \step{3}). 
Finally, we compare the machine codes of the variants embedded in a single module to make sure that they are different (Step \step{4}). 
If they are not, this means the compilation chain has removed what made them unique and we discard this module from our experiment. 
It should be noted that we use the most aggressive optimizations possible with Cranelift so that we are keeping the modules where we are sure that the variants are preserved. 

To provide an even better understanding of our pipeline, let us analyze the example in the diagram. Hypothetically, CROW generates 2 variants for the original module in \step{1}. Rustc compiles the 2 bytecode modules, generating 2 unique Wasm packages \step{2}. Two symmetric pairs can be built \step{3} from the 2 generated Wasm binaries. Then, for each pair, the Cranelift compiler generates the corresponding machine code. In one pair, the generated machine codes are equal even when the original pair is formed by two different Wasm codes so we discard it \step{4}. For the other, the generated machine codes are different and we keep it. In the end, we have a 50\% preservation rate as variants in one module out of two were preserved.  


\todo{Fix table,  x86 instead of machine code}


For each module inside the projects, we perform the workflow described in \autoref{diagram:methodrq1}. We collect all the Wasm variant pairs for the diversified functions inside the module. We then calculate the preservation rate on the generated x86 machine code with Cranelift. 



%Assumptions:

%- The analysis phase can be done from everywhere, So, moving target network wont work, since the application is deployed in a world scale. Besides, the main idea of the Edge is to get rid of the latency, this technique will increase the latency.

%- Since the platform is heterogeneous, there is a natural protection according to Holland \etal. But it is not enough

%- FaaS is small enough to embed the multiversion in the same binary

%- The model attack is a combination C of parameters that can trigger a bad behavior. The developer does not know C, then, C should not work for all nodes. If developer already know C, the combination should not work more than one time between the discovery and the successful redeployment.

%- The removal of latency, allows the study of time side-channel close to the client. \todo{Check !}. If there is time side-channel attacks, check that the generated diversification is less than the natural latency and greater than the lapse between regional classification.


\begin{comment}
 

\lstdefinestyle{nccode}{
    numbers=none,
    firstnumber=2,
    stepnumber=1,
    numbersep=10pt,
    tabsize=4, 
    showspaces=false,
    breaklines=true, 
    showstringspaces=false,
    moredelim=**[is][\btHL]{`}{`},
    moredelim=**[is][{\btHL[fill=black!10]}]{`}{`},
    moredelim=**[is][{\btHL[fill=celadon!40]}]{!}{!}
}
\lstset{
    language=WAT,
    style=nccode,
    basicstyle=\footnotesize\ttfamily,
    columns=fullflexible,
    breaklines=true
}
\begin{code}
\noindent\begin{minipage}[b]{0.9\linewidth}
    \captionof{lstlisting}{Constant operand splitting.}\label{add:prevalence_example}
    \noindent\rule{\linewidth}{0.4pt}
    \begin{minipage}[t]{0.45\linewidth}
        \begin{lstlisting}
i32.const 9                                           
i32.add                                                
i32.const 4                                          
i32.add                                               
i32.const 12                                        
i32.add                                              
i32.const 7                                     å     
i32.add  
        \end{lstlisting}
    \end{minipage}%
    \hfill\noindent\begin{minipage}[t]{0.45\linewidth}
       
        \begin{lstlisting}
i32.const 13
i32.add
i32.const 8
i32.add
i32.const 1
i32.add
i32.const 10
i32.add
        \end{lstlisting}
    \end{minipage}
\end{minipage}
\end{code}


\begin{code}
\noindent\begin{minipage}[b]{0.9\linewidth}
    \captionof{lstlisting}{Inversion of operations.}\label{add:prevalence_example}
    \noindent\rule{\linewidth}{0.4pt}
    \begin{minipage}[t]{0.45\linewidth}
        \begin{lstlisting}
i32.const -<n>
i32.sub
        \end{lstlisting}
    \end{minipage}%
    \hfill\noindent\begin{minipage}[t]{0.45\linewidth}
       
        \begin{lstlisting}
i32.const <n>
i32.add
        \end{lstlisting}
    \end{minipage}
\end{minipage}
\end{code}



\begin{code}
\noindent\begin{minipage}[b]{0.9\linewidth}
    \captionof{lstlisting}{Multiplication overflow.}\label{add:prevalence_example}
    \noindent\rule{\linewidth}{0.4pt}
    \begin{minipage}[t]{0.45\linewidth}
        \begin{lstlisting}
  i32.const -1931544174
  i32.mul
  i32.const 109653155
  i32.mul
        \end{lstlisting}
    \end{minipage}%
    \hfill\noindent\begin{minipage}[t]{0.45\linewidth}
       
        \begin{lstlisting}
  i32.const -10
  
  
  i32.mul
        \end{lstlisting}
    \end{minipage}
\end{minipage}
\end{code}





\begin{code}
\noindent\begin{minipage}[b]{0.9\linewidth}
    \captionof{lstlisting}{Multiplication overflow.}\label{add:prevalence_example}
    \noindent\rule{\linewidth}{0.4pt}
    \begin{minipage}[t]{0.45\linewidth}
        \begin{lstlisting}
  i32.const -1931544174
  i32.mul
  i32.const 109653155
  i32.mul
        \end{lstlisting}
    \end{minipage}%
    \hfill\noindent\begin{minipage}[t]{0.45\linewidth}
       
        \begin{lstlisting}
  i32.const -10
  
  
  i32.mul
        \end{lstlisting}
    \end{minipage}
\end{minipage}
\end{code}


\end{comment}

\subsection{Definitions (to be removed)}
In this subsection we define the key concepts for that we use along the paper. 

\todo{Define on the fly.}
\todo{Define multivariant call graph in term of variants and dispatchers.}

\begin{definition}{Unique Wasm variants, $W(F)$:}\label{def:W}
    Let $F$ be a program function, $W(F)$ a set of Wasm binaries  such that each binaryis a unique function variant generated by CROW from a function $F$.
\end{definition}

\begin{definition}{Binary translation function ,$C$:}\label{def:compiler}
    Let $w$ be a Wasm module, $x$ an x86 machine code and $C: Wasm \rightarrow x86 $ a translation function. $C$ is a binary translation function if it generates the corresponding x86 machine code $x$ for the Wasm binary$w$ such that $C(w) = x$.
\end{definition}

\begin{definition}{Unique x86 variants , $X(F)$:}\label{def:X}
    Let $F$ be a function, $W$ the Unique Wasm variants set according to \autoref{def:W} and $C$ a compiler function according to \autoref{def:compiler}. We define $X$ = \{ $x, C(w) = x, w \in W$ \} as the set of unique x86 machines codes that can be generated from $W$.
\end{definition}



\begin{definition}{Multivariant binary:}\label{def:EP}
    Let $F$ a function and $W$ its collection of variants. The multivariant binary $M$ is the binarythat packages all function variants in it. Notice that the concept of multivariant could be applied to any code representation. We use multivariant binary indistinctly for any code representation, for example, " multivariant Wasm  binary".
\end{definition}

\begin{definition}{Call Graph (CG):}\label{def:EP}
    We use an approximation of the traditional definition of Call Graph from Aho \etal \citationneeded. We only take into account the functions that executes in a static analysis of the source code. 
\end{definition}

\begin{definition}{Execution traces:}\label{def:DEP}
    Let $F$ an endpoint function in the Edge service. The execution path $S = F_1, F_2, ... F_n$ is the trace of the function in the Call Graph of the binary, executed from the request to the response to the client. 
\end{definition}



In 2019, it was accepted as the fourth official language for the web \cite{WebAssemblyCoreSpecification}.
Moreover, \wasm is used in standalone environments beyond the web context \cite{2021arXiv210212730N, 1244493Jacobsson, WARDuino2019,eWenWasmachine,10.1145/3423211.3425680}.
Nowadays, languages such as C/C++, C\#, Go and Rust can be compiled to Wasm \cite{hilbig2021empirical}. 
Since version 9.0, LLVM added the \wasm backend as a platform for code generation, making possible the generation of Wasm code from any LLVM frontend.

\begin{metric}{Deployment speed:}\label{metric:size}
For a given binary, the time passed between uploading the binary to the Fastly Edge infrastructure to its deployment to the edge nodes is the deployment time. 
We measure the deployment time for both kind of binaries, original and multivariant.
\end{metric}

% Define deployment time
Since the deployment time is correlated with the size of the binary, we collect Metric \autoref{metric:size} only for the largest multivariant binary.
The largest multivariant binary is generated for the endpoint \textbf{generate\_qr\_str}.
The original and multivariant binaries have 3Mb and 13Mb of size respectively.

% How to collect the times
We collect 500 deployment times for each.
To avoid the possible jitter in the network, we collect the deployment time from 4 different edge nodes in 4 different timezones.
The total number of collected deployment times is $2\times 4\times 500$.

\todo{TBD, should we mention the protocol to collect the deplyment time ? }


% Worst case
The largest size of a multivariant binary is 13Mb for the original binary named \textbf{generate\_qr\_str}, which has a size of 3Mb.
In this case, the deployment time is increased by approx. 1 second from the original mean deployment time of 12.07s.
These values are in concordance with the average time reported by Fastly for its deployment time, which is 13s.
Therefore, the deployment time is not increased by the multivariant binaries created by \tool.


%\todo{Add A Stackelberg Game and Markov Modeling of Moving Target Defense as well }\url{https://www.researchgate.net/publication/320203887_A_Stackelberg_Game_and_Markov_Modeling_of_Moving_Target_Defense}
%\todo{https://arxiv.org/pdf/1905.13293.pdf}

%The main difference with currently available MTD systems is that \tool performs the multivariant system in an automated way. 


%Serverless approaches

% Standalone interpreters for \wasm

% \todo{Add aWsm paper here as   a previous work for Sledge}



%\todo{ wasmachine -> Virtual machine execution for wearables based on
%WebAssembly. \cite{1244493Jacobsson} }




%Benchmark studies, feasibility and Wasm in Edge approaches%

%This is more a motivation to the usage of Wasm

%\todo{Considering WebAssembly Containers for Edge Computing on Hardware-Constrained IoT Devices 2020 master thesis Blekinge \cite{Napieralla2020}.}





% 2014



%Torquato, Matheus, and Marco Vieira. "Moving target defense in cloud computing: A systematic mapping study." Computers & Security 92 (2020): 101742.


%\todo{TBD, multivariatn execution means to execute several variants at the same time to detect anomalies. 
%}

%\textbf{Moving Target Defense and security related}



We collect $64\times100$ execution traces because the deplyment speed of our experimentation platform is in average 13s. 
In an hypothetical case of attack, if it detected a patch or even the disconnection of the service can be done in 13s.
This makes unreallistic to collect the traces in more than 13s.

\subsection{Moving Target Defense}

\todo{purpose of these two paragraphs is not clear. Do we need a subsection about MTD?}



\lstset{
    language=CURL,
    style=nccode,
    basicstyle=\footnotesize\ttfamily,
    columns=fullflexible,
    breaklines=true
}

\begin{code}
\noindent\begin{minipage}[b]{0.9\linewidth}
    
    \begin{minipage}[t]{1\linewidth}
        \begin{lstlisting}
< HTTP/2 200 
< xpop: BMA
< xpophash: 1293274507
< xtime: 1999109
!< xpath: !
! [1859, 1836, 1765, 1767, 1800, 1767, 1801, !
! 1767, 1799, 1767, 1800, 1767, 1801, 1767, !
! 1801, 1767, 1801, 1767, 1800, 1767, 1799, !
! 1767, 1800, 1767, 1799, 1767, 1799, 1767, !
! 1801, 1767, 1799, 1767, 1801, 1767, 1799, !
! 1767, 1799, 1767, 1801, 1767, 1800, 1767, !
! 1799, 1767, 1801, 1767, 1801, 1767, 1799, !
! 1767, 1801, 1767, 1799, 1767, 1800, 1767, 1801]!
< date: Thu, 03 Jun 2021 14:33:36 GMT
< content-length: 74
< 
{ [74 bytes data]
* Connection #0 to host totally-devoted-krill.edgecompute.app left intact
* Closing connection 0
        \end{lstlisting}
    \end{minipage}%
    
    \noindent\rule{\linewidth}{0.4pt}
    \captionof{lstlisting}{Execution path retrieval example for one query to one of the executed endpoints. The execution path is highlighted in the header of the response in green color. Each function is annotated with an unique id.}\label{retrieval_example}
\end{minipage}
\end{code}


\todo{the end of the paragraph is very hard to understand}
This cloud model \todo{what is 'this cloud model'?} is done at or near the customer’s physical location instead of relying on the cloud at one of a dozen data centers to do all the work. 
Literally, this has a geographic meaning. 
Every time an Edge endpoint is executed, the closest node is the one responding.

\todo{how is this first sentence related to the previous paragraph?}


\todo{Javier: TBD, lets avoid to talk about security here}
% Swivel and Spectre
On the other hand, even when \wasm is a performant way to deploy services at the Edge \cite{10.1145/3302505.3310084}, Narayan \etal \cite{2021arXiv210212730N} remarked, it is not exempt of vulnerabilities.
Spectre attacks can bypass Wasm's isolation.
A malicious deployed Wasm can use Spectre to break out of the sandbox to leak another process memory by miss-training the speculative execution of the Edge node CPU.
v


\begin{figure}
    \includegraphics[width=0.8\linewidth]{diagrams/RQ1.pdf}
    \caption{Example of a Multivariant Call Graph and its preservation during x86 compilation. From left to right: original binary CG, Wasm multivariant binary MCG generated by \tool and the x86 multivariant binary MCG that is deployed after Lucet compiles the Wasm multivariant to machine code.}
    \label{diag:rq1}
\end{figure}


Machine learning models can be deployed to the Edge for faster classification near to devices \cite{https://doi.org/10.1002/spe.2944}.
These models are not exempt of vulnerabilities.
Roy \etal \cite{10.1145/3318216.3363338} proposed a moving target defense against adversarial machine learning.
Their technique shows that switching among machine learning algorithms can be used to defend against boundedly rational adversary without sacrificing performance.
In addition, they remarked that adding more randomness to the algorithm variants achieve better defense.
\tool adds a remarkable amount if different execution paths in an automated way that a multivariant Wasm module can execute and can be used to increment of uncertainty for adversarial-based attacks.



\subsection{RQ2 Results. Compile-time diversity preservation}
% Sum again the methodology
We translate each \wasm multivariant binary with Lucet, to determine the impact of this translation to machine code on the function variants and the diversity of paths in the multivariant call graph. 

% Description of the table and general stats
The 'x86 code' section of \autoref{table:CFG1} summarizes the key data to answer RQ2. Column \#Variants shows the number of preserved variants in the x86 code of each endpoint, column \#Paths shows the number of possible paths in the x86 multivariant binary. The last two columns show  the ratio of paths (PP) and variants (PV) preserved in x86. 
Note that the path preservation ratio metric is a projection of the variant preservation and the call graph in the multivariant binary.

 
% Previous works and why some functions have several preserved transformations
In all cases, more than 77\% of the individual function variants present in the multivariant Wasm binary are preserved in the x86 multivariant. This high preservation rate for function variants allows to preserve a large ratio of possible paths in the multivariant call graph.
In 4 out of 7 cases, more than 83\% of the possible execution paths in the multivariant Wasm  binary are preserved.
The translation to machine code preserves 21\% and 17\% of the possible paths for \texttt{qr\_str} and \texttt{qr\_image}. Yet, the x86 version of the multiversion call graph for these endpoints still includes millions of possible paths, with 17 and 15 randomization points. The translation to machine drastically reduces the potential for randomized execution paths only for \texttt{bin2base64}, for which it preserves only 25\% of the possible paths, for a total of 41 paths.

% Population's compression
We have identified why some variants are not preserved the translation from Wasm to x86. Lucet performs optimization passes before generating machine code. 
In some cases, this can annihilate the effect of CROW's diversification transformation. 
For example, in \autoref{mul:prevalence_example}, CROW synthesizes a variant in the right column by splitting it in two  multiplications relying on the integer overflow mechanism. 
A  constant merging optimization pass could remove the constant multiplications by performing it at compilation time. 
The other transformation cases that we have observed have the same property, the transformations are simple enough to be quickly verified at compilation time.

\lstset{
    language=WAT,
    style=WATStyle,
    stepnumber=0,
    label=EQExample}
\begin{code}
\noindent\begin{minipage}[b]{0.9\linewidth}
    
    \begin{minipage}[t]{0.45\linewidth}
        \begin{lstlisting}
; previous stack code;
i32.const -10
i32.mul
        \end{lstlisting}
    \end{minipage}%
    \hfill\noindent\begin{minipage}[t]{0.45\linewidth}
       
        \begin{lstlisting}
; previous stack code ;
i32.const -1931544174
i32.mul
i32.const 109653155
i32.mul
        \end{lstlisting}
    \end{minipage}
    
    \noindent\rule{\linewidth}{0.4pt}
    \captionof{lstlisting}{Two examples of block variants that are functionally equivalent and implement with different \wasm instructions. The variant on the left, generated by \tool, is not preserved through the translation to machine code.}\label{mul:prevalence_example}
\end{minipage}
\end{code}





We identified where the optimizations are done in Lucet's compiler, \footnote{\url{https://github.com/bytecodealliance/wasmtime/blob/main/cranelift/codegen/src/preopt.peepmatic} and \url{https://github.com/bytecodealliance/wasmtime/blob/main/cranelift/codegen/src/postopt.rs}}. It performs optimization-like transformations that are simpler than the ones introduced by CROW. 
With this result we also encourage to avoid the usage of the insertion of \texttt{nop} instructions either in Wasm or machine code. \texttt{nop} operations could be easily detected and removed by a latter optimization stage.



Moreover, the last three endpoints have a path preservation ratio that is less than 0.25, even with more than 87\%  of individual function  variants that are preserved. This is explained by the fact that the number of possible paths is related to both the number of variants and to the complexity of the call graph.

{
\begin{figure}
    \begin{center}
        \includegraphics[width=\linewidth]{diagrams/example_cfg.pdf}
    \end{center}
    
    \caption{ From top to bottom: original binary call graph,  multivariant \wasm  binary call graph generated by \tool and the  multivariant x86 binary call graph resulting from Lucet's compilation to x86 machine code. This example illustrates that if only variant is not preserved through the translation to x86, the number of paths significantly decreases}
    \label{diag:preservation}
\end{figure}
}



The example in \autoref{diag:preservation}  illustrates this phenomenon.
Suppose an original binary composed of three functions with the call graph illustrated at the top of the figure. Here, we count 2 possible paths (one with no iteration, and one with a single iteration).
\tool generates 2 variants for $f2$ and 4 variants for $f3$, the multivariant wasm call graph is illustrated at the center of the figure. The number of possible execution paths increases to 40.
In the translation process, Lucet transforms the two \wasm function variants for $f2$ into the same x86 function.
In this case, the number of possible execution paths in the x86 multivariant call graph is reduced by a factor of 2, from 40 to 20.
However, the number of variants is decreased only in 1. 
The complexity of the call graph has a major impact on the number of possible execution paths. 


\begin{tcolorbox}[title=Answer to RQ2]
     The translation from \wasm to machine code through Lucet preserves a high ratio of function variants. This leads to the preservation of high numbers of possible execution paths in the multivariant binaries. 
     Our multivariant execution scheme is appropriate for the state-of-the-art runtime of edge computing nodes.
\end{tcolorbox}

%In the following we list and describe the observed cases where the transformation pairs are not preserved.


==> tables/execution.tex <==
{\small
\begin{table}
%\setlength\minrowclearance{1.0pt}
\renewcommand{\arraystretch}{0.9}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\centering
%\resizebox{\linewidth}{!}{
\begin{tabular}{ l | r | r | r | r }
    \midrule
    Function & \#Unique traces & \#Pairs & \#Unique Pairs & DTW distrib \\
    \hline
    \textbf{libsodium} & \\
    \hline
    f7 & 100 & 100$\times$100 & 100$\times$100 & \includegraphics[width=20mm]{plots/t.pdf} \\
    f3 & 100 & 100$\times$100 & 100$\times$100 & \includegraphics[width=20mm]{plots/t.pdf} \\
    f5 & 100 & 100$\times$100 & 100$\times$100 & \includegraphics[width=20mm]{plots/t.pdf} \\
    f10 & 100 & 100$\times$100 & 100$\times$100 & \includegraphics[width=20mm]{plots/t.pdf} \\
    TODO bin2base64
\end{tabular}
%}

\caption{ }\label{table:intra_mtd}
\end{table}
}

==> tables/execution_times.bck.tex <==

\definecolor{celadon}{rgb}{0.67, 0.88, 0.69}
{
\begin{table}
%\setlength\minrowclearance{1.0pt}
\small
\centering
%\resizebox{\linewidth}{!}{
\begin{tabular}{  p{1.5cm}  r r | r r}
    & \multicolumn{2}{c|}{\textbf{Original bin.}} & \multicolumn{2}{c}{\textbf{Multivariant Wasm bin.}} \\
    \hline
    Endpoint & Median(ns) & $\sigma$ & Median(ns) & $\sigma$ \\
    \hline
    \hline
    
    \textbf{libsodium}  \\
    \hline
    
encrypt  & 7976 & 5263 & 217341 & 43905 \\

decrypt  & 13175 & 6508 & 225529 & 47786 \\

random  & 16511 & 7857 & 232509 & 53713 \\

invert  & 119917 & 34721 & 341420 & 65830 \\

bin2base64  & 10751 & 5373 & 215253 & 35315 \\

\hline
\textbf{qrcode-rust} \\
\hline
qr\_str & 3117575 & 418539 & 492606388 & 36864122 \\
qr\_image & 3091728 & 412912 & 512669965 & 41718087 \\
\hline

\end{tabular}
%}
\caption{Execution time for the original endpoints and its multivariants. The table is structured in two sections. The first section shows the endpoint name, the median execution time and its standard deviation for the original endpoint. The second section shows the median execution time and its standard deviation for the multivariant \wasm binary.}\label{table:ex_times}
\end{table}
}


==> tables/pops_table.tex <==
{\footnotesize
\begin{table*}
%\setlength\minrowclearance{1.0pt}
\renewcommand{\arraystretch}{1.1}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\centering
%\resizebox{\linewidth}{!}{
\begin{tabular}{ l r | l r | l r | l r   }
    \midrule
    POP code & Machines count & POP code & Machines count & POP code & Machines count & POP code & Machines count \\
    \hline
    \hline
 CPH &  3 & MXP &  11 & CGH &  60 & BUR &  54 \\ \hline
 EZE &  4 & HND &  30 & PAO &  51 & DAL &  63 \\ \hline
 STL &  29 & CMH &  31 & LCY &  49 & SEA &  62 \\ \hline
 GIG &  10 & EWR &  58 & LON &  55 & LGA &  64 \\ \hline
 BMA &  6 & LCK &  4 & BOS &  63 & DUB &  6 \\ \hline
 BWI &  62 & WDC &  62 & MRS &  61 & MSP &  83 \\ \hline
 MCI &  32 & CHI &  62 & ORD &  20 & MAD &  31 \\ \hline
 ITM &  38 & HKG &  6 & PDK &  60 & YYZ &  19 \\ \hline
 BOM &  19 & OSL &  4 & HHN &  55 & DEN &  61 \\ \hline 
 SJC &  57 & FTY &  62 & HEL &  5 & MAN &  29 \\ \hline
 DEL &  18 & VIE &  6 & IAH &  58 & AKL &  10 \\ \hline 
 PWK &  60 & MIA &  67 & SYD &  23 & MDW &  62 \\ \hline
 LHR &  62 & JNB &  4 & MEL &  37 & SCL &  4 \\ \hline
 FRA &  62 & MAA &  19 & GRU &  18 & AMS &  56 \\ \hline 
 STP &  8 & TYO &  94 & DCA &  59 & CDG &  59 \\ \hline
 DFW &  64 & BOG &  5 & LAX &  65 & YUL &  13 
\end{tabular}
%}
\caption{Number of computers per POP}\label{table:pops}
\end{table*}
}

==> tables/single_case_mcg.tex <==

\definecolor{celadon}{rgb}{0.67, 0.88, 0.69}
{
\begin{table}
%\setlength\minrowclearance{1.0pt}
\renewcommand{\arraystretch}{0.9}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\centering
%\resizebox{\linewidth}{!}{
\begin{tabular}{  p{5cm} |  r  }
    \midrule
    Endpoint & \# Wasm variants  \\
    \hline
    \hline
    
    \textbf{libsodium}  \\
    \hline
\textbf{...chacha20poly1305\_ietf\_decrypt...} & 27 \\
crypto\_verify\_n & 77 \\
...chacha20\_ietf\_xor\_ic & 9 \\
\end{tabular}
%}

\caption{Number of variants for functions involved in the Multivariant Call Graph of the ...chacha20poly1305\_ietf\_decrypt... endpoint. }\label{table:stability_single_case}
\end{table}
}

\todo{Move the table to a text explanation}

==> tables/stabilit3.tex <==

\definecolor{celadon}{rgb}{0.67, 0.88, 0.69}
{
\begin{table}
%\setlength\minrowclearance{1.0pt}
\renewcommand{\arraystretch}{0.9}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\centering
%\resizebox{\linewidth}{!}{
\begin{tabular}{  p{6cm}   r }
    \midrule
    Endpoint &  |Wasm MCG| \\
    \hline
    
    \textbf{libsodium}  \\
    \hline
    
...chacha20poly1305\_ietf\_decrypt... & 18711 \\

...ed25519\_scalar\_random & 12635 \\

sodium\_bin2base64 & 3780  \\

...ed25519\_scalar\_invert & 2660 \\

...chacha20poly1305\_ietf\_encrypt... & 216  \\


\end{tabular}
%}

\caption{Multivariant Call Graph sizes for libsodium .... The table is structured as follows: project name, endpointfunction name, size of Multivariant Call Graph for the multivariant Wasm binary corresponding with the endpoint. The rows are sorted by the size of the MCG.}\label{table:mcg1}
\end{table}
}

\todo{Merge the two tables}

==> tables/stability.bck.tex <==
{\small
\begin{table*}
%\setlength\minrowclearance{1.0pt}
\renewcommand{\arraystretch}{1.1}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\centering
%\resizebox{\linewidth}{!}{
\begin{tabular}{ l | r | r | r | r }
    \midrule
    Module name & Unique Wasm & Total pairs compared & Reversed Pairs & Metric 1 \\
    \hline
    \hline
    utils & 199 & 19701 & 12793 & 35.06\% \\
    \hline
    aead\_xchacha20poly1305 & 171 & 14535 & 0 & 100.00\% \\
    \hline
    secretbox\_xchacha20poly1305 & 148 & 10878 & 3568 & 67.20\% \\
    \hline
    pwhash\_scryptsalsa208sha256 & 123 & 7503 & 2269 & 69.76\% \\
    \hline
    crypto\_secretbox\_easy & 108 & 5778 & 1602 & 72.27\% \\
    \hline
    ed25519\_ref10 & 56 & 1540 & 24 & 98.44\% \\
    \hline
    verify & 43 & 903 & 112 & 87.60\% \\
    \hline
    pbkdf2-sha256 & 26 & 325 & 56 & 82.77\% \\
    \hline
    stream\_salsa208\_ref & 22 & 231 & 99 & 57.14\% \\
    \hline
    pwhash\_scryptsalsa208sha256\_nosse & 22 & 231 & 1 & 99.57\% \\
    \hline
    argon2 & 21 & 210 & 0 & 100.00\% \\
    \hline
    salsa20\_ref & 19 & 171 & 70 & 59.06\% \\
    \hline
    codecs & 19 & 171 & 0 & 100.00\% \\
    \hline
    blake2b-long & 17 & 136 & 0 & 100.00\% \\
    \hline
    randombytes\_internal\_random & 13 & 78 & 1 & 98.72\% \\
    \hline
    hash\_sha512\_cp & 10 & 45 & 0 & 100.00\% \\
    \hline
    hash\_sha256\_cp & 10 & 45 & 0 & 100.00\% \\
    \hline
    stream\_salsa2012\_ref & 10 & 45 & 12 & 73.33\% \\
    \hline
    generichash\_blake2b & 8 & 28 & 0 & 100.00\% \\
    \hline
    core\_salsa\_ref & 7 & 21 & 0 & 100.00\% \\
    \hline
    shorthash\_siphashx24\_ref & 7 & 21 & 0 & 100.00\% \\
    \hline
    core\_hsalsa20\_ref2 & 6 & 15 & 0 & 100.00\% \\
    \hline
    x25519\_ref10 & 5 & 10 & 1 & 90.00\% \\
    \hline
    shorthash\_siphash24\_ref & 4 & 6 & 0 & 100.00\% \\
    \hline
    core\_hchacha20 & 4 & 6 & 0 & 100.00\% \\
    \hline
    crypto\_scrypt-common & 4 & 6 & 0 & 100.00\% \\
    \hline
    aead\_chacha20poly1305 & 3 & 3 & 0 & 100.00\% \\
    \hline
    auth\_hmacsha512 & 3 & 3 & 0 & 100.00\% \\
    \hline
    scalarmult\_ristretto255\_ref10 & 3 & 3 & 0 & 100.00\% \\
    \hline
    auth\_hmacsha256 & 3 & 3 & 0 & 100.00\% \\
    \hline
    obsolete & 2 & 1 & 0 & 100.00\% \\
    \hline
    pwhash\_argon2id & 2 & 1 & 0 & 100.00\% \\
    \hline
    pwhash\_argon2i & 2 & 1 & 0 & 100.00\% \\
    \hline
    keypair & 2 & 1 & 0 & 100.00\% \\
    \hline
     \textbf{Sum} & 1317 & 85657 & 20612 & 75.94\%
\end{tabular}
%}
\caption{Transformation stability}\label{table:stability}
\end{table*}
}

==> tables/stability.tex <==
{\small
\begin{table*}
%\setlength\minrowclearance{1.0pt}
\renewcommand{\arraystretch}{0.9}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\centering
%\resizebox{\linewidth}{!}{
\begin{tabular}{ l l | r | r | r }
    \midrule
    Module name & Function & Unique Wasm & Total Pairs compared  & Metric 1 \\
    \hline
    \hline
ed25519\_ref10 & & & & \\
 & fe25519\_isnegative & 427 & 90951 & 99.94 \%\\
 & ge25519\_scalarmult & 260 & 33670 & 99.69 \%\\
 & fe25519\_tobytes & 80 & 3160 & 100.00 \%\\
\hline
argon2-fill-block-ref  & & & & \\
 & init\_block\_value & 472 & 111156 & 99.97 \%\\
 & xor\_block & 20 & 190 & 99.47 \%\\
 & fBlaMka & 16 & 120 & 100.00 \%\\
 & rotr64 & 4 & 6 & 100.00 \%\\
 & fill\_block & 2 & 1 & 100.00 \%\\
\hline
utils & & & & \\
 & \textbf{sodium\_increment} & 118 & 6903 & 99.29 \%\\
 & \textbf{sodium\_memcmp} & 102 & 5151 & 99.38 \%\\
 & \textbf{sodium\_is\_zero} & 95 & 4465 & 99.51 \%\\
 & \textbf{sodium\_add} & 50 & 1225 & 97.39 \%\\
 & sodium\_free & 35 & 595 & 100.00 \%\\
 & \_unprotected\_ptr\_from\_user\_ptr & 27 & 351 & 99.72 \%\\
 & sodium\_pad & 14 & 91 & 100.00 \%\\
 & \_sodium\_malloc & 8 & 28 & 100.00 \%\\
 & sodium\_compare & 6 & 15 & 100.00 \%\\
 & \_sodium\_alloc\_init & 2 & 1 & 100.00 \%\\
\hline
x25519\_ref10 & & & & \\
 & crypto\_scalarmult\_curve25519\_ref10\_base & 123 & 7503 & 97.71 \%\\
 & fe25519\_cswap & 103 & 5253 & 99.49 \%\\
 & has\_small\_order & 59 & 1711 & 99.24 \%\\
 & fe25519\_add & 28 & 378 & 100.00 \%\\
 & crypto\_scalarmult\_curve25519\_ref10 & 13 & 77 & 100.00 \%\\
 & fe25519\_sub & 4 & 6 & 100.00 \%\\
\hline
obsolete & & & & \\
 & crypto\_sign\_edwards25519sha512batch\_keypair & 230 & 26335 & 98.49 \%\\
 & crypto\_sign\_edwards25519sha512batch\_open & 52 & 1326 & 93.29 \%\\
\hline
core\_ed25519 & & & & \\
 & \textbf{crypto\_core\_ed25519\_scalar\_random} & 133 & 8778 & 99.83 \%\\
 & \textbf{crypto\_core\_ed25519\_scalar\_complement} & 81 & 3240 & 99.75 \%\\
 & \textbf{crypto\_core\_ed25519\_scalar\_invert} & 28 & 378 & 99.74 \%\\
\hline
argon2-core & & & & \\
 & argon2\_initialize & 80 & 3159 & 99.87 \%\\
 & store\_block & 79 & 3081 & 99.87 \%\\
 & xor\_block & 4 & 6 & 100.00 \%\\
 & argon2\_fill\_first\_blocks & 3 & 3 & 66.67 \%\\
 & clear\_memory & 2 & 1 & 100.00 \%\\
 & allocate\_memory & 2 & 1 & 100.00 \%\\
\hline
blake2b-ref & & & & \\
 & blake2b\_init\_param & 54 & 1431 & 99.86 \%\\
 & blake2b\_is\_lastblock & 27 & 351 & 99.72 \%\\
 & blake2b\_init0 & 16 & 120 & 99.17 \%\\
 & blake2b\_update & 3 & 3 & 100.00 \%\\
 & blake2b\_salt\_personal & 2 & 1 & 100.00 \%\\
 & blake2b\_init\_key\_salt\_personal & 2 & 1 & 100.00 \%\\
 & blake2b & 2 & 1 & 100.00 \%\\
\hline
codecs & & & & \\
 & \textbf{sodium\_bin2base64} & 42 & 861 & 99.88 \%\\
 & b64\_byte\_to\_char (not usable internal linking) & 30 & 435 & 99.77 \%\\
 & sodium\_bin2hex & 7 & 21 & 100.00 \%\\
 & b64\_urlsafe\_char\_to\_byte & 3 & 3 & 66.67 \%\\
 & b64\_char\_to\_byte & 3 & 3 & 66.67 \%\\
 & b64\_byte\_to\_urlsafe\_char & 3 & 3 & 66.67 \%\\
\hline
pwhash\_scryptsalsa208sha256\_nosse & & & & \\
 & integerify & 48 & 1128 & 97.07 \%\\
 & blkcpy & 16 & 120 & 99.17 \%\\
 & blockmix\_salsa8 & 15 & 105 & 99.05 \%\\
\hline
verify & & & & \\
 & crypto\_verify\_n & 77 & 2926 & 98.84 \%\\
\hline
aead\_xchacha20poly1305 & & & & \\
 & \_decrypt\_detached & 34 & 561 & 100.00 \%\\
 & \_encrypt\_detached & 33 & 528 & 100.00 \%\\
\hline
\end{tabular}
%}
\caption{Transformation stability}\label{table:stability}
\end{table*}
}

==> tables/stability2.tex <==
{\small
\begin{table*}
%\setlength\minrowclearance{1.0pt}
\renewcommand{\arraystretch}{0.9}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\centering
%\resizebox{\linewidth}{!}{
\begin{tabular}{ l l | r | r | r }
    \midrule
    Module name & Function & Unique Wasm & Total Pairs compared  & Metric 1 \\
    \hline
    \hline
aead\_chacha20poly1305 & & & & \\
 & \textbf{crypto\_aead\_chacha20poly1305\_ietf\_decrypt\_detached} & 27 & 351 & 100.00 \%\\
 & \textbf{crypto\_aead\_chacha20poly1305\_ietf\_encrypt\_detached} & 24 & 276 & 100.00 \%\\
 & crypto\_aead\_chacha20poly1305\_ietf\_decrypt & 3 & 3 & 66.67 \%\\
 & crypto\_aead\_chacha20poly1305\_decrypt & 2 & 1 & 100.00 \%\\
\hline
argon2-encoding & & & & \\
 & u32\_to\_string (not usable, internal) & 32 & 496 & 99.60 \%\\
 & argon2\_encode\_string (not usable, hidden) & 22 & 230 & 99.57 \%\\
\hline
secretbox\_xsalsa20poly1305 & & & & \\
 & crypto\_secretbox\_xsalsa20poly1305 & 18 & 153 & 98.69 \%\\
 & crypto\_secretbox\_xsalsa20poly1305\_open & 3 & 3 & 66.67 \%\\
\hline
chacha20\_ref & & & & \\
 & stream\_ref\_xor\_ic & 20 & 190 & 58.42 \%\\
\hline
pbkdf2-sha256 & & & & \\
 & escrypt\_PBKDF2\_SHA256 & 17 & 136 & 99.26 \%\\
\hline
pwhash\_scryptsalsa208sha256 & & & & \\
 & pickparams & 9 & 36 & 97.22 \%\\
 & crypto\_pwhash\_scryptsalsa208sha256\_str & 2 & 1 & 100.00 \%\\
\hline
crypto\_secretbox\_easy & & & & \\
 & crypto\_secretbox\_open\_detached & 4 & 6 & 100.00 \%\\
 & crypto\_secretbox\_detached & 4 & 6 & 100.00 \%\\
 & crypto\_secretbox\_open\_easy & 3 & 3 & 66.67 \%\\
\hline
core\_salsa\_ref & & & & \\
 & rotl32  & 10 & 45 & 100.00 \%\\
\hline
core\_hsalsa20\_ref2 & & & & \\
 & rotl32 & 10 & 44 & 100.00 \%\\
\hline
stream\_chacha20 & & & & \\
 & crypto\_stream\_chacha20\_ietf\_xor\_ic & 9 & 36 & 100.00 \%\\
\hline
secretbox\_xchacha20poly1305 & & & & \\
 & crypto\_secretbox\_xchacha20poly1305\_detached & 4 & 6 & 100.00 \%\\
 & crypto\_secretbox\_xchacha20poly1305\_open\_detached & 4 & 6 & 100.00 \%\\
\hline
poly1305\_donna & & & & \\
 & poly1305\_finish & 4 & 6 & 100.00 \%\\
 & poly1305\_blocks & 4 & 6 & 100.00 \%\\
\hline
crypto\_box\_easy & & & & \\
 & crypto\_box\_open\_easy & 3 & 3 & 66.67 \%\\
 & crypto\_box\_open\_easy\_afternm & 3 & 3 & 66.67 \%\\
\hline
box\_curve25519xchacha20poly1305 & & & & \\
 & crypto\_box\_curve25519xchacha20poly1305\_open\_easy & 3 & 3 & 66.67 \%\\
 & crypto\_box\_curve25519xchacha20poly1305\_open\_easy\_afternm & 3 & 3 & 66.67 \%\\
\hline
pwhash\_argon2i & & & & \\
 & \_needs\_rehash & 3 & 3 & 66.67 \%\\
 & crypto\_pwhash\_argon2i\_str & 2 & 1 & 100.00 \%\\
\hline
open & & & & \\
 & crypto\_sign\_ed25519\_open & 5 & 10 & 70.00 \%\\
\hline
argon2 & & & & \\
 & argon2\_hash & 3 & 3 & 100.00 \%\\
 & argon2\_verify & 2 & 1 & 100.00 \%\\
\hline
box\_seal\_curve25519xchacha20poly1305 & & & & \\
 & crypto\_box\_curve25519xchacha20poly1305\_seal\_open & 3 & 3 & 66.67 \%\\
\hline
pwhash\_argon2id & & & & \\
 & crypto\_pwhash\_argon2id\_str\_verify & 2 & 1 & 100.00 \%\\
\hline
blake2b-long & & & & \\
 & blake2b\_long & 2 & 1 & 100.00 \%\\
\hline
 &  & & 329992 & 99.63 \%\\

\end{tabular}
%}
\caption{Diversification preservation: static diversity}\label{table:stability}
\end{table*}
}

\todo{Add real unique after compilation in the table}

==> tables/stability4.tex <==

\definecolor{celadon}{rgb}{0.67, 0.88, 0.69}
{\small
\begin{table}
%\setlength\minrowclearance{1.0pt}
\renewcommand{\arraystretch}{0.9}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\centering
%\resizebox{\linewidth}{!}{
\begin{tabular}{  l  r  r  r  }
    \midrule
    Endpoint & |Wasm MCG | & |x86 MCG| & Ratio \\
    \hline

    \textbf{libsodium}  \\
    \hline
    
...chacha20poly1305\_ietf\_encrypt... & 216 & 216 & 1.00 \\

...ed25519\_scalar\_invert & 2660 & 2106 & 0.79 \\

...chacha20poly1305\_ietf\_decrypt... & 18711 & 13851 & 0.74 \\

...ed25519\_scalar\_random & 12635 & 9360 & 0.74 \\

sodium\_bin2base64 & 3780 & 2378 & 0.63  \\
\end{tabular}
%}

\caption{Multivariant Call Graph preservation for libsodium .... The table is structured as follows: project name, function name, size of the Wasm Multivariant Call Graph, size of the x86 machine code Multivariant Call Graph and the relative size. The rows are sorted by the relative size of the Multivariant Call Graphs}\label{table:stability}
\end{table}
}

==> tables/stability_cyclomatic.tex <==

\definecolor{celadon}{rgb}{0.67, 0.88, 0.69}
{
\begin{table}
%\setlength\minrowclearance{1.0pt}
\renewcommand{\arraystretch}{0.9}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\centering
%\resizebox{\linewidth}{!}{
\begin{tabular}{  p{3.8cm}  r r r r }
    \midrule
    Endpoint & Original &  Wasm & x86 & Ratio \\
    \hline
    
    \textbf{libsodium}  \\
    \hline
    
...chacha20poly1305\_ietf\_encrypt... & 16 & 62 & 57 & 0.91 \\

...chacha20poly1305\_ietf\_decrypt... & 15 & 132 & 127 & 0.96 \\

...ed25519\_scalar\_random & 4 & 230 & 227 & 0.98 \\

...ed25519\_scalar\_invert & 7 & 128 & 126 & 0.99\\

sodium\_bin2base64 & 2 & 53 & 42 & 0.79 \\



\end{tabular}
%}

\caption{Multivariant Call Graph sizes for libsodium .... The table is structured as follows: project name, endpointfunction name, size of Multivariant Call Graph for the multivariant Wasm binary corresponding with the endpoint. The rows are sorted by the size of the MCG.}\label{table:CFG1}
\end{table}
}



==> tables/stability_paths.bck.tex <==

\definecolor{celadon}{rgb}{0.67, 0.88, 0.69}
{
\begin{table}
%\setlength\minrowclearance{1.0pt}
\renewcommand{\arraystretch}{0.9}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\centering
%\resizebox{\linewidth}{!}{
\begin{tabular}{  p{2.2cm}  r r r  r | r r }
    \midrule
    Endpoint & \#Original &  \#Wasm  & \#x86 & Ratio & \#F & \#D \\
    \hline
    
    \textbf{libsodium}  \\
    \hline
    
...chacha20poly1305\_ietf\\$\hookrightarrow$ \_encrypt... & 4 & 325 & 253 & 0.83 & 5 \\

...chacha20poly1305\_ietf\\$\hookrightarrow$\_decrypt... & 3 & 84 & 78 & 0.93 & 4 \\

...ed25519\_scalar\_random & 2 & 12864 & 12314 & 0.96 & 1 \\

...ed25519\_scalar\_invert & 1 & 2784 & 2538 & 0.91 & 1\\

sodium\_bin2base64 & 1 & 172 & 41 & 0.25 & 1 \\

\hline
\textbf{qrcode-rust} \\
\hline
generate\_qr\_str & ~7M & ~100M & ~20M & 0.21 & 17 \\
generate\_qr\_image & ~1M & ~3M & 617K & 0.17 & 15 \\
\hline

\end{tabular}
%}

\caption{Possible execution paths for the studied projects. The table is structured as follows: project name, endpoint function name, possible execution paths for the original module, possible execution paths for the Wasm multivariant module, posible execution paths for the x86 multivariant module, the ratio between them and the number of created dispatchers. The rows are sorted by the number of possible execution paths in the original module.}\label{table:CFG1}
\end{table}
}



==> tables/stability_single_case.tex <==

\definecolor{celadon}{rgb}{0.67, 0.88, 0.69}
{\small
\begin{table}
%\setlength\minrowclearance{1.0pt}
\renewcommand{\arraystretch}{0.9}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\centering
%\resizebox{\linewidth}{!}{
\begin{tabular}{  l  r | r  }
    \midrule
    Entry & \#Wasm & \#x86  \\
    \hline
    \hline
    
    \textbf{libsodium}  \\
    \hline
\textbf{...chacha20poly1305\_ietf\_decrypt...} & 27 & 27 \\
crypto\_verify\_n & 77 & 57\\
...chacha20\_ietf\_xor\_ic & 9 & 9\\
\hline
Size of the static function call graph & 18711 & 13851 \\

\end{tabular}
%}

\caption{Single function entry point example from libsodium. }\label{table:stability_single_case}
\end{table}
}
